Secure and Fast Asynchronous Vertical Federated Learning via Cascaded Hybrid Optimization

Vertical Federated Learning (VFL) attracts increasing attention because it empowers multiple parties to jointly train a privacy-preserving model over vertically partitioned data. Recent research has shown that applying zeroth-order optimization (ZOO) has many advantages in building a practical VFL algorithm. However, a vital problem with the ZOO-based VFL is its slow convergence rate, which limits its application in handling modern large models. To address this problem, we propose a cascaded hybrid optimization method in VFL. In this method, the downstream models (clients) are trained with ZOO to protect privacy and ensure that no internal information is shared. Meanwhile, the upstream model (server) is updated with first-order optimization (FOO) locally, which significantly improves the convergence rate, making it feasible to train the large models without compromising privacy and security. We theoretically prove that our VFL framework converges faster than the ZOO-based VFL, as the convergence of our framework is not limited by the size of the server model, making it effective for training large models with the major part on the server. Extensive experiments demonstrate that our method achieves faster convergence than the ZOO-based VFL framework, while maintaining an equivalent level of privacy protection. Moreover, we show that the convergence of our VFL is comparable to the unsafe FOO-based VFL baseline. Additionally, we demonstrate that our method makes the training of a large model feasible.

==> A4a_ConvergenceAanlysisWithProofSketch.tex <==
\section{Convergence Analysis} \label{sec:convergence}
    \subsection{Theoretical Difficulty}
        The theoretical difficulty of our work comes from the cascaded hybrid optimization in the VFL, where different optimization methods are simultaneously applied to the upstream and downstream parts of the VFL. 
        To the best of our knowledge, all related works in VFL have only considered a single type of optimization method in the entire VFL during one iteration, whose analytic result can be more easily derived via the same analytic steps on the entire framework. 
        However, our work required different analytic procedures to be applied to different parts of the model to solve the problem, which posed a significant challenge. 
        Specifically, the analytic procedure for ZOO and FOO is vastly different, making it difficult to analyze these two different optimizations in one model.


    \subsection{Assumptions}
        % Assumptions. 
        Assumptions \ref{assum:feasible_optimal_solution} - \ref{assum:bounded_variance} are the basic assumptions for solving the non-convex optimization problem with stochastic gradient descent \cite{ghadimi2013stochastic, liu2019communication, zhang2021desirable}. Assumption~\ref{assum:feasible_optimal_solution} tells that the global minima $f^*$ is not $-\infty$~\cite{ghadimi2013stochastic, liu2018zeroth, zhang2021desirable}. Assumption~\ref{assum:smoothness} is used for modeling the smoothness of the loss function $f(\cdot)$, with which we can link the difference of the gradients with the difference of the input in the definition domain. Assumption~\ref{assum:unbiased_gradient} is a common assumption for stochastic gradient descent telling that the expectation of the estimation of the stochastic gradient of the sample $i$ does not have a systematic error or bias~\cite{ghadimi2013stochastic}. Assumption~\ref{assum:bounded_variance} tells that the variance of the gradient estimation is bounded~\cite{liu2018zeroth}. 
        
        \begin{assumption}\label{assum:feasible_optimal_solution}
        {\bf{Feasible Optimal Solution:}} Function $f$ is bounded below that is, there exist $f^*$ such that,
        \begin{align}
            f^*:=\inf_{[w_0,{{\bw }}]\in \mathbb{R}^d} f(w_0,{{\bw}}) > -\infty. \nonumber
        \end{align}
        \end{assumption}
        \begin{assumption}\label{assum:smoothness}
             {\textbf{Lipschitz Gradient:}} $\nabla f_i$ is $L$-Lipschitz continuous w.r.t. all the parameter, i.e., there exists a constant $L$ for $ \forall \ [w_0,{{\bf w}}], [w_0', {{\bf w}}']$  such that
            \begin{align}
                & \norm{ \nabla_{[w_0,{{\bf w}}]} f_i (w_0, \bw) - \nabla_{[w_0,{{\bf w}}]} f_i (w'_0, \bw')} \NN 
                & \qquad \qquad\qquad\qquad \le L \norm{[w_0,{{\bf w}}]-[w_0',{{\bf w}}']} \nonumber
            \end{align}
            specifically there exists an $L_m>0$ for all parties $m=0,\cdots,M$ such that $\nm f_i$ is $L_m$-Lipschitz continuous:
            \begin{align} 
                    & \norm{ \nm f_i (w_0,\bw) - \nm f_i (w_0',\bw')} \NN 
                    & \qquad \qquad\qquad\qquad \le L_m \norm{[w_0,{{\bf w}}]-[w_0',{{\bf w}}']} \nonumber
            \end{align}
        \end{assumption}
        
        \begin{assumption}\label{assum:unbiased_gradient}
            {\textbf{Unbiased Gradient:}} For $m \in 0, 1, \cdots M $ for every data sample $i$, the stochastic partial derivatives for all participants are unbiased, i.e.  
                $$ \BE[i] \nm f_i(w_0, \bw ) = \nm \f{w_0, \bw} $$
        \end{assumption}
    
        \begin{assumption}\label{assum:bounded_variance}
            \textbf{Bounded Variance:} For  $ m = 0, 1, \cdots, M $, there exist constants $\sigma_m \le \infty $ such that the variance of the stochastic partial derivatives are bounded: 
                $$\BE[i] \norm{\nm f_i(w_0, \bw) - \nm f(w_0, \bw) }^2 \leq \sigma_m^2 $$
        \end{assumption}
    
        Assumption~\ref{assum:bounded_embedding_gradients} is a common assumption for analyzing VFL when bounding some terms for the entire model when the rest parts have been bounded \cite{castiglia2022compressed, gu2021privacy, zhang2021secure}. We only apply this assumption in the parts of convergence analysis that do not affect the analytic result. 
        \begin{assumption}\label{assum:bounded_embedding_gradients}
            \textbf{Bounded Block-coordinate Gradient:} The gradient w.r.t. all the client is bounded, i.e. there exist positive constants $\mathbf{G}_m$ for the client $ m = 1, \cdots, M $ the following inequalities hold: 
            \begin{align}
                \norm{ \nm \hm(\wm; x_{m, i}) } \le \mG_m  \nonumber
            \end{align}
        \end{assumption}
    
        % Asynchronous Update. 
        Assumption~\ref{assum:independent_client}-\ref{assum:bound_delay} are fundamental and widely used assumptions for analyzing the asynchronous VFL~\cite{zhang2021desirable, chen2020vafl, gu2021privacy}. 
        Asynchronous updates introduce delays for clients when calculating losses. 
        We assume that the activation of clients at each global round is independent (assumption~\ref{assum:independent_client}) and that the maximum delay is bounded (assumption~\ref{assum:bound_delay}), which are reasonable assumptions for modeling asynchronous VFL. 
        Without a bounded delay assumption, convergence cannot be achieved, and the convergence result cannot be further simplified because the distribution of client activation is unknown.
        
        \begin{assumption}\label{assum:independent_client} {\bf{Independent Client:}}
            The activated client $m_t$ for the global iteration $t$ is independent of $m_0$, $\cdots,$ $m_{t-1}$ and satisfies $\mathbb{P}(m_t=m):=p_m$
        \end{assumption}
        
        \begin{assumption}\label{assum:bound_delay}{\bf{Uniformly Bounded Delay:}} For each client $m$, and each sample $i$, the delay at each global iteration $t$ is bounded by a constant $\tau$. i.e. $\tau_{m, i}^t \le \tau $
        \end{assumption} 

    \subsection{Theorems}
        \begin{theorem} \label{theo:1}
            Under assumption \ref{assum:feasible_optimal_solution} - \ref{assum:bound_delay}, to solve the problem \ref{eq:problem} with algorithm \ref{algo:1} the following inequality holds.
            \begin{align} %\label{eq:result-2}
                            & \frac{1}{T } \sumt \BE \normsq{\nabla \f{w_0^{t}, \bw^{t}} }  \NN
                \leos{}     & \frac{4\ps \BE \bigp{f^0 - f^*}}{T \eta} + \eta \bigp{ 4 \ps \Ls \sigma_*^2 + 8 \ps \Ls \ds \sigma_*^2 + \ps \Ls^3 \mus^2 \ds^2}\NN
                            & + \eta^2\bigp{ 18 \ps \tau^2  \Ls^2 \ds \mGs^2 + 5 \ps \tau^2 \Ls^2 \mus^2 \Ls^2 \ds^2 }  + \mus^2\bigp{\ps \Ls^3 \ds^2}\nonumber
            \end{align}
            where $\Ls = \max_m \bigcb{L, L_0, L_m}$, $ \ds = \max_m \bigcb{ d_{m} } $, $\eta_0 = \eta_m = \eta \le \frac{1}{4 \Ls \ds}$, $\frac{1}{\ps} = \min_m p_m $, $\mus = \max_m \bigcb{\mu_m} $, $\mGs = \max_m \bigcb{\mG_m}$, and $T$ is the number of iterations. 
        \end{theorem}
        
        \begin{remark}
            Theorem~\ref{theo:1} tells that the major factors that affect the convergence are the learning rate $\eta$, the smoothing coefficient $\mu$ for the ZOO, and the biggest parameter size $\ds$ among the clients.  
        \end{remark}
    
        \begin{corollary} \label{coro:1}
            If we choose $\eta = \frac{1}{\sqrt{T}}$, $ \mu = \frac{1}{\sqrt{T}}$, we can derive 
            \begin{align}
                        &   \frac{1}{T} \sumt \BE \normsq{\nabla \f{w_0^{t}, \bw^{t}} }  \NN
            \leos{}     &   \frac{1}{\sqrt{T}} \bigsb{ 4\ps \BE \bigp{f^0 - f^*} +  4 \ps \Ls \sigma_*^2 + 8 \ps \Ls \ds \sigma_*^2 } \NN
                        & + \frac{1}{T}\bigp{ 18 \ps \tau^2  \Ls^2 \ds \mGs^2 + 5 \ps \tau^2 \mus^2 \Ls^4 \ds^2 + \ps  \Ls^3 \ds^2} \NN  
                        & + \frac{1}{T^\frac{3}{2}} \bigp{ \ps \Ls^3 \ds^2 } \nonumber
            \end{align}
            where the parameters are the same as that in Theorem~\ref{theo:1}.
            
        \end{corollary}
    
        \begin{remark}
            Corollary~\ref{coro:1} demonstrates the convergence of our cascaded hybrid optimization framework and shows that it converges in $\mathcal{O}\bigp{\frac{d_*}{\sqrt{T}}} $, where $d_* = \underset{m}{\max} \bigcb{d_{m}}$ represents the largest model size among the clients, and $T$ denotes the number of iterations.
        
            %\begin{align}
            %    \frac{1}{T} \sumt \BE \normsq{\nabla \f{w_0^{t}, \bw^{t}} } = \mathcal{O}\bigp{\frac{d}{\sqrt{T}}} \nonumber
            %\end{align}
        \end{remark}
        
        \begin{remark}
            Comparing our convergence analysis result and ZOO-VFL~\cite{zhang2021desirable}, our result does not include the parameter size of the server ($d_0$) in the constant terms, which demonstrates that the convergence of the global model is not limited by the size of the server's parameter. Therefore, in our framework, the server can apply a larger model without impacting the convergence of the global model. 
        \end{remark}
        




==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
